BizBench: A Quantitative Reasoning Benchmark for Business and Finance

Answering questions within business and finance requires reasoning, precision, and a wide-breadth of technical knowledge. Together, these requirements make this domain difficult for large language models (LLMs). We introduce BizBench, a benchmark for evaluating models' ability to reason about realistic financial problems. BizBench comprises eight quantitative reasoning tasks, focusing on question-answering (QA) over financial data via program synthesis. We include three financially-themed code-generation tasks from newly collected and augmented QA data. Additionally, we isolate the reasoning capabilities required for financial QA: reading comprehension of financial text and tables for extracting intermediate values, and understanding financial concepts and formulas needed to calculate complex solutions. Collectively, these tasks evaluate a model's financial background knowledge, ability to parse financial documents, and capacity to solve problems with code. We conduct an in-depth evaluation of open-source and commercial LLMs, comparing and contrasting the behavior of code-focused and language-focused models. We demonstrate that the current bottleneck in performance is due to LLMs' limited business and financial understanding, highlighting the value of a challenging benchmark for quantitative reasoning within this domain.

==> table-model.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
%     \hline
%     {\bf Name} & {\bf \#Tokens} & {\bf \#Params} & {\bf Compute} \\
%     & {\bf (B)} & {\bf (B)} & \\ \hline
%     \hline
%     MPT         & 1,000 & 7         & \\
%     MPT         & 1,000 & 30        &  \\
%     \hline
%     Falcon      & 1,000 & 7         &  \\
%     Falcon      & 1,000 & 40        &  \\
%     \hline
%     StarCoder   & 1,000 & 15.5      &  \\
%     \hline
%     LLaMa 2     & 2,000 & 7         &  \\
%     LLaMa 2     & 2,000 & 13        &  \\
%     LLaMa 2     & 2,000 & 70        &  \\
%     \hline
%     CodeLlaMa   & 2,500 & 7         &  \\
%     CodeLlaMa   & 2,500 & 13        &  \\
%     CodeLlaMa   & 2,500 & 34        &  \\
%     \hline
%     FinLM       & 500   & 13        &  \\
%     FinLM       & 1,000 & 30        &  \\
    
%     \hline
%     GPT-3        & 300 & 175       &  \\
%     GPT-3.5      & 300* & 175       &  \\
%     GPT-4        & 13,000* & -      &  \\
%     \hline
% \end{tabular}
% }
% \caption{Evaluation models.}
% \label{tab:model}
% \end{table}

==> table-template.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c}
%        Tasks  & Template \\
%        Extraction tasks  & \\
%             % Context:
%             % {context}
%             % Question: {question}
%             % Python Program:
%             % {program}
%        Code Synthesis & \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:template}
% \end{table*}
